Detecting Textual Adversarial Examples through Randomized Substitution and Vote

A line of work has shown that natural text processing models are vulnerable to adversarial examples. Correspondingly, various defense methods are proposed to mitigate the threat of textual adversarial examples, eg, adversarial training, input transformations, detection, etc. In this work, we treat the optimization process for synonym substitution based textual adversarial attacks as a specific sequence of word replacement, in which each word mutually influences other words. We identify that we could destroy such mutual interaction and eliminate the adversarial perturbation by randomly substituting a word with its synonyms. Based on this observation, we propose a novel textual adversarial example detection method, termed Randomized Substitution and Vote (RS&V), which votes the prediction label by accumulating the logits of k samples generated by randomly substituting the words in the input text with synonyms. The proposed RS&V is generally applicable to any existing neural networks without modification on the architecture or extra training, and it is orthogonal to prior work on making the classification network itself more robust. Empirical evaluations on three benchmark datasets demonstrate that our RS&V could detect the textual adversarial examples more successfully than the existing detection methods while maintaining the high classification accuracy on benign samples.

==> figs/adb_vote.tex <==
\begin{figure}[tb]
\centering
\includegraphics[width=\linewidth]{figs/pdf/ag_news_vote.pdf}
\caption{The restore accuracy (\%) of \name using various values of vote num $k$ where 
random rate $p$ is fixed to 60 on CNN model on AG's News under Textfooler attack}
\label{fig:abd_vote}
\end{figure}
